Learning-Enabled Robust Control with Noisy Measurements

We present a constructive approach to bounded $\ell_2$-gain adaptive control with noisy measurements for linear time-invariant scalar systems with uncertain parameters belonging to a finite set. The gain bound refers to the closed-loop system, including the learning procedure. The approach is based on forward dynamic programming to construct a finite-dimensional information state consisting of $\mathcal H_\infty$-observers paired with a recursively computed performance metric. We do not assume prior knowledge of a stabilizing controller.

==> figures/closed_loop_explicit_noise.tex <==
\begin{tikzpicture}[node distance = 6em, line width=0.5mm, inner ysep=6pt, >=latex]
	\node [block, align = center] (sys) {Linear system with \\ uncertain parameters};

	\node[block, above of = sys, align = center] (delta) {Unmodelled \\ dynamics};
	\node[block, below of = sys, align = center] (controller) {Learning-Enabled \\ Robust Controller};
	
	\node[left =8em of sys] (out) {};
	\node[right = 8em of sys]  (in) {};

	\node[coordinate, right = 3em of sys, yshift=-1em] (Cout) {};
	\node[coordinate, left =3em of sys, yshift=-1em] (Cin) {};

	\node[coordinate, right = 3em of sys, yshift=1em] (Dout) {};
	\node[coordinate, left =3em of sys, yshift=1em] (Din) {};

	\node[block, below = 1.5 em of Cin] (sensor) {Sensor};
	%\node[below left = 0.5em and 0.5em of Cin, align=center] () {noisy \\ measurements};
	\coordinate[left = 3em of sensor] (noise) {};


	\draw[->] (in) -- node[pos=0.15, label={disturbances}] () {} (sys);
	\draw[->] (sys) -- node[pos=0.85, label={errors}]() {} (out);
	\draw[->] ([yshift=-1em]sys.west) -- (Cin) -- (sensor);
	\draw[->] (sensor) |- (controller);
	\draw[->] ([yshift=1em]sys.west) -- (Din) |- (delta);
	\draw[<-] ([yshift=-1em]sys.east) -- (Cout) |- (controller);
	\draw[<-] ([yshift=1em]sys.east) -- (Dout) |- (delta);
	\draw[->] (noise) -- node[label={noise}] () {} (sensor);
\end{tikzpicture}

